DDANet: Dual Decoder Attention Network for Automatic Polyp Segmentation

Colonoscopy is the gold standard for examination and detection of colorectal polyps. Localization and delineation of polyps can play a vital role in treatment (e.g., surgical planning) and prognostic decision making. Polyp segmentation can provide detailed boundary information for clinical analysis. Convolutional neural networks have improved the performance in colonoscopy. However, polyps usually possess various challenges, such as intra-and inter-class variation and noise. While manual labeling for polyp assessment requires time from experts and is prone to human error (e.g., missed lesions), an automated, accurate, and fast segmentation can improve the quality of delineated lesion boundaries and reduce missed rate. The Endotect challenge provides an opportunity to benchmark computer vision methods by training on the publicly available Hyperkvasir and testing on a separate unseen dataset. In this paper, we propose a novel architecture called ``DDANet'' based on a dual decoder attention network. Our experiments demonstrate that the model trained on the Kvasir-SEG dataset and tested on an unseen dataset achieves a dice coefficient of 0.7874, mIoU of 0.7010, recall of 0.7987, and a precision of 0.8577, demonstrating the generalization ability of our model.

==> takeouts.tex <==
% 
%We aim to develop an accurate and robust method for surgical instrument segmentation from endoscopic images based on computer vision techniques. However, one of the significant problem in the field is lack of publicly available dataset for benchmarking the algorithms and improving the benchmark on the same datasets\cite{jha2020kvasir}. For the Kvasir-instrument dataset, we have used UNet architecture, which is common semantic segmentation based architecture for medical image segmentation tasks. Next, we provide a baseline algorithm that provides and invite multimedia researcher to improve the baseline methods. In this paper, we present our approach for binary instrument segmentation on the endoscopic instrument segmentation dataset. 


%Semantic segmentation is a well known task in the computer vision community, its aim is to label each image pixel with a specified class. It  helps you to understand the  content and  to recognize objects in an  image. It is used widely in remote sensing, autonomous driving, medical image analysis and many more. In biomedical domain semantic segmentation has be widely used to analyze a different type of image data such as the X-rays, CT, MRI, Endoscopy imaging, Fundus imaging and many more. It helps  to  understand the structure of a complex image data and easy diagnosis of  a variety of medical conditions including pneumonia, cancer, etc. One such cancer is colorectal cancer which one of the leading cause of death worldwide.

%Semantic segmentation is the task of understanding the scene in an image by predicting the class label for each pixel. Such scene understanding is crucial for many computer-vision based applications, such as remote sensing, autonomous driving, medical image analysis and many more. However, the ability to predict the class label for each pixel is a challenging task in itself. In medical image analysis, semantic segmentation helps in the diagnosis of the underlying disease by understanding the region which is affected by the disease, thus enabling effective diagnosis.

%The current state-of-the-art models for the semantic segmentation are trained continuously on the dataset that is given to them. They don't take into account the information that the model is learning in every epoch and try to use that information along with the dataset to train the model. In every epoch, the model learns some new information and we can use that information along with the dataset in the next epoch and try to get better model performance by repeating this learning process in every epoch.


%Medical image segmentation is a key task in clinical applications which helps to identify boundaries of the lesions such as abnormal regions (for instance, sessile polyps) inside colon in the image. Since manual labeling is time consuming, tedious, error-prone, and subjective process, an automatic \ac{CADx} system can be of crucial significance both for clinicians are researchers. The segmentation results can provide detail information about the location of the lesions and it can be helpful for treatment, planning and therapy. 

%Advances in medical imaging technology (such as endoscopy, X-ray, MRI, Ultrasound, wireless capsule endoscopy) and others have revolutionized the way of handling the anatomical and pathological events inside the body. In computer vision, \ac{CNN} have shown remarkable success even for semantic segmentation task.


We use the semantic segmentation on the polyp dataset provided by the challenge organizer for automatic polyp segmentation. We used a dual decoder network sharing a common encoder, where we predicted the segmentation mask and the original input image in the grayscale format. Along with the segmentation branch, we also build an autoencoder branch. We use the feature maps from the autoencoder branch to provide attention to the segmentation branch. To further improve the performance, we use a squeeze and excitation network with the residual block.
 
 
 
%In the polyp image segmentation task (binary segmentation task), precision shows over-segmentation, and recall shows under-segmentation. Thus, we also encourage to calculate precision and recall.

%For \textit{automatic polyp segmentation task}, \textbf{mIoU} is used for evaluation and ranking of the teams. There is a direct correlation between mIoU and DSC. Therefore, we have only used one metric.

% In the polyp image segmentation task (binary segmentation task), precision shows over-segmentation, and recall shows under-segmentation. Thus, we also encourage to calculate precision and recall.

% For \textit{automatic polyp segmentation task}, \textbf{mIoU} is used for evaluation and ranking of the teams. There is a direct correlation between mIoU and DSC. Therefore, we have only used one metric.

% Till here!

%Challenges are formal platforms to invite researchers working to address the same problem. By inviting the multiple participants, we provide an opportunity to the researchers to evaluate current state-of-the-art algorithm on the same dataset. Thus, through this year's Medico challenge, we challenge the participants on the Kvasir-SEG dataset to develop more efficient algorithms and solve the polyp segmentation task. 



% In this paper, we propose a novel deep learning architecture, called \ac{DDANet} for automatic polyp segmentation. The dual decoder network shares a common endocer, where we predict the segmentation mask and the original input image in the grayscale format for performance improvement. In the proposed network, along with the segmentation branch, we also build an autoencoder branch. We use the feature maps from the autoencoder branch to  generate an attention map, which is used with the segmentation branch to enhance the important features.
% First paragraph here!


    %\and
    %NIHR Oxford Biomedical Research Centre, Oxford University Hospitals NHS Foundation Trust, Oxford, UK
    
    
    %\author{Blinded}
%\authorrunning{Blinded et al.}
%\institute{Blinded}


% Q: this should be reconstruction, you wont get the same image????  check

%The encoder takes the RGB image as input which passes through the shared encoder. The encoder gradually downsamples the input and create an abstract representation of the image using different encoder blocks. After that, both the decoders uses this abstract representation, where the first tries to reconstruct the segmentation mask and the second decoder gives the input image in the grayscale format. 

%  \begin{table}[t]
%  \caption{Quantitative results provided by the organizers on unseen dataset.}
%     \label{table:testdatset}
%     \def\arraystretch{1.5}
%      \setlength\tabcolsep{3pt}
%     \par\bigskip
%     \centering
%   \begin{tabular}{l|l|l|l|l}
% \hline
% \textbf{Method} & \textbf{DSC} & \textbf{mIOU} & \textbf{Recall} & \textbf{Precision}  \\ \hline

% \end{tabular}
% \end{table} 

%However, we cannot show similar qualitative results on the unseen dataset (test dataset provided by organizers) as we do not have the output prediction masks. 
